mlirSynth: Automatic, Retargetable Program Raising in Multi-Level IR using Program Synthesis

MLIR is an emerging compiler infrastructure for modern hardware, but existing programs cannot take advantage of MLIR's high-performance compilation if they are described in lower-level general purpose languages. Consequently, to avoid programs needing to be rewritten manually, this has led to efforts to automatically raise lower-level to higher-level dialects in MLIR. However, current methods rely on manually-defined raising rules, which limit their applicability and make them challenging to maintain as MLIR dialects evolve. We present mlirSynth -- a novel approach which translates programs from lower-level MLIR dialects to high-level ones without manually defined rules. Instead, it uses available dialect definitions to construct a program space and searches it effectively using type constraints and equivalences. We demonstrate its effectiveness \revi{by raising C programs} to two distinct high-level MLIR dialects, which enables us to use existing high-level dialect specific compilation flows. On Polybench, we show a greater coverage than previous approaches, resulting in geomean speedups of 2.5x (Intel) and 3.4x (AMD) over state-of-the-art compilation flows for the C programming language. mlirSynth also enables retargetability to domain-specific accelerators, resulting in a geomean speedup of 21.6x on a TPU.

==> algorithms/synthesis.tex <==
\begin{algorithmic}
  \Function{Synthesise}{function}
  \State $args \gets \text{genRandomArgs}(function.args)$
  \State $targetValue \gets \text{execute}(function, args)$
  \State $activeSet \gets \text{initCandidates}(function)$
  \State $operations \gets \text{pickOperations}(function)$
  \While{true}
  \For{$op$ \textbf{in} $operations$}
  \State $operands \gets activeSet$
  \State $attributes \gets \text{genAttrs}(op.attrTypes)$
  \State $regions \gets \text{genRegions}(op.regionTypes)$
  \For{$candidate$ \textbf{in} \text{cartesianProduct}(operands, attributes, regions)}
  \If{not verify(candidate)}
  \State \textbf{continue}
  \EndIf
  \State $value \gets \text{execute}(candidate, args)$
  \If{$value = targetValue$}
  \State \textbf{return} $candidate$
  \EndIf
  \If{not unique(activeSet, value)}
  \State \textbf{continue}
  \EndIf
  \State $activeSet \gets activeSet \cup {\text{candidate}}$
  \EndFor
  \EndFor
  \EndWhile
  \EndFunction

  \Function{initCandidates}{function}
  \State $candidates \gets \text{set()}$
  \State $candidates \gets candidates \cup function.arguments$
  \State $candidates \gets candidates \cup \text{simpleConstants}$
  \State \textbf{return} $candidates$
  \EndFunction
\end{algorithmic}

